The Merging Path Plot: adaptive fusing of k-groups with likelihood-based model selection

There are many statistical tests that verify the null hypothesis: the variable of interest has the same distribution among k-groups. But once the null hypothesis is rejected, how to present the structure of dissimilarity between groups? In this article, we introduce The Merging Path Plot - a methodology, and factorMerger - an R package, for exploration and visualization of k-group dissimilarities. Comparison of k-groups is one of the most important issues in exploratory analyses and it has zillions of applications. The classical solution is to test a~null hypothesis that observations from all groups come from the same distribution. If the global null hypothesis is rejected, a~more detailed analysis of differences among pairs of groups is performed. The traditional approach is to use pairwise post hoc tests in order to verify which groups differ significantly. However, this approach fails with a large number of groups in both interpretation and visualization layer. The~Merging Path Plot methodology solves this problem by using an easy-to-understand description of dissimilarity among groups based on Likelihood Ratio Test (LRT) statistic.

==> article_init <==
\begin{thebibliography}{18}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[B<b6>ck(2014)]{atools}
A.~B<b6>ck.
\newblock \emph{Atools: Atools}, 2014.
\newblock URL \url{https://R-Forge.R-project.org/projects/biostat/}.
\newblock R package version 0.2/r191.

\bibitem[Bondell and Reich(2008)]{Casanova}
H.~D. Bondell and B.~J. Reich.
\newblock {Simultaneous factor selection and collapsing levels in ANOVA}.
\newblock \emph{Department of Statistics, North Carolina State University},
  2008.

\bibitem[Cox(1992)]{coxph}
D.~R. Cox.
\newblock Regression models and life-tables.
\newblock In \emph{Breakthroughs in statistics}, pages 527--541. Springer,
  1992.

\bibitem[Czepiel(2002)]{binom}
S.~A. Czepiel.
\newblock Maximum likelihood estimation of logistic regression models: theory
  and implementation.
\newblock \emph{Available at czep. net/stat/mlelr. pdf}, 2002.

\bibitem[{de Mendiburu}(2016)]{Agric}
F.~{de Mendiburu}.
\newblock \emph{agricolae: Statistical Procedures for Agricultural Research},
  2016.
\newblock URL \url{https://CRAN.R-project.org/package=agricolae}.
\newblock R package version 1.2-4.

\bibitem[Fox and Weisberg(2011)]{car}
J.~Fox and S.~Weisberg.
\newblock \emph{An {R} Companion to Applied Regression}.
\newblock Sage, Thousand Oaks {CA}, second edition, 2011.
\newblock URL \url{http://socserv.socsci.mcmaster.ca/jfox/Books/Companion}.

\bibitem[Friedman et~al.(2001)Friedman, Hastie, and
  Tibshirani]{friedman2001elements}
J.~Friedman, T.~Hastie, and R.~Tibshirani.
\newblock \emph{The elements of statistical learning}, volume~1.
\newblock Springer series in statistics Springer, Berlin, 2001.

\bibitem[Genz and Bretz(2009)]{mvtnorm}
A.~Genz and F.~Bretz.
\newblock \emph{Computation of Multivariate Normal and t Probabilities}.
\newblock Lecture Notes in Statistics. Springer-Verlag, Heidelberg, 2009.
\newblock ISBN 978-3-642-01688-2.

\bibitem[Hothorn et~al.(2008)Hothorn, Bretz, and Westfall]{Multcomp}
T.~Hothorn, F.~Bretz, and P.~Westfall.
\newblock Simultaneous inference in general parametric models.
\newblock \emph{Biometrical Journal}, 50\penalty0 (3):\penalty0 346--363, 2008.

\bibitem[Lenth(2016)]{lsmeans}
R.~V. Lenth.
\newblock Least-squares means: The {R} package {lsmeans}.
\newblock \emph{Journal of Statistical Software}, 69\penalty0 (1):\penalty0
  1--33, 2016.
\newblock \doi{10.18637/jss.v069.i01}.

\bibitem[Maj et~al.(2013)Maj, Prochenka, and Pokarowski]{DMR}
A.~Maj, A.~Prochenka, and P.~Pokarowski.
\newblock \emph{DMR: Delete or Merge Regressors for linear model selection.},
  2013.
\newblock URL \url{https://CRAN.R-project.org/package=DMR}.
\newblock R package version 2.0.

\bibitem[Prochenka(2016)]{Proch}
A.~Prochenka.
\newblock \emph{{Delete or Merge Regressors algorithm}}, chapter 4.3, 5--6,
  pages 37, 44--91.
\newblock 2016.

\bibitem[{Terry M. Therneau} and {Patricia M. Grambsch}(2000)]{survival-book}
{Terry M. Therneau} and {Patricia M. Grambsch}.
\newblock \emph{Modeling Survival Data: Extending the {C}ox Model}.
\newblock Springer, New York, 2000.
\newblock ISBN 0-387-98784-3.

\bibitem[Tibshirani et~al.(2005)Tibshirani, Saunders, Rosset, Zhu, and
  Knight]{Tib}
R.~Tibshirani, M.~Saunders, S.~Rosset, J.~Zhu, and K.~Knight.
\newblock {Sparsity and smoothness via the fused lasso}.
\newblock \emph{Journal of the Royal Statistical Society}, pages 01--108, 2005.

\bibitem[Tukey(1949)]{Tukey}
J.~Tukey.
\newblock {Comparing Individual Means in the Analysis of Variance}.
\newblock \emph{BIOMETRICS}, pages 99--114, 1949.

\bibitem[Venables and Ripley(2002)]{MASS}
W.~N. Venables and B.~D. Ripley.
\newblock \emph{Modern Applied Statistics with S}.
\newblock Springer, New York, fourth edition, 2002.
\newblock URL \url{http://www.stats.ox.ac.uk/pub/MASS4}.
\newblock ISBN 0-387-95457-0.

\bibitem[Wickham(2009)]{ggplot2}
H.~Wickham.
\newblock \emph{ggplot2: Elegant Graphics for Data Analysis}.
\newblock Springer-Verlag New York, 2009.
\newblock ISBN 978-0-387-98140-6.
\newblock URL \url{http://ggplot2.org}.

\bibitem[Wilks(1938)]{wilks1938large}
S.~S. Wilks.
\newblock The large-sample distribution of the likelihood ratio for testing
  composite hypotheses.
\newblock \emph{The Annals of Mathematical Statistics}, 9\penalty0
  (1):\penalty0 60--62, 1938.

\end{thebibliography}

